Data-dependent kernels in nearly-linear time

We propose a method to efficiently construct data-dependent kernels which can make use of large quantities of (unlabeled) data. Our construction makes an approximation in the standard construction of semi-supervised kernels in Sindhwani et al. 2005. In typical cases these kernels can be computed in nearly-linear time (in the amount of data), improving on the cubic time of the standard construction, enabling large scale semi-supervised learning in a variety of contexts. The methods are validated on semi-supervised and unsupervised problems on data sets containing upto 64,000 sample points.

==> bibcommands.tex <==

%bibliography papers

\newcommand{\WeightedMajorityTwo}{DBLP:journals/iandc/LittlestoneW94}

%semi-supervised learning
\newcommand{\MeasureBased}{DBLP:conf/nips/BousquetCH03}
\newcommand{\ZhangSemisupervised}{ZhangO00}
\newcommand{\CastellicoverMixing}{DBLP:journals/tit/CastelliC96}
\newcommand{\CastelliCoverExponentialValue}{DBLP:journals/prl/CastelliC95}
\newcommand{\BlumMitchellCoTraining}{Blum1998}
\newcommand{\RatsabySemisupervised}{DBLP:conf/colt/RatsabyV95}
\newcommand{\NigamText}{DBLP:conf/aaai/NigamMTM98}
\newcommand{\ZhuGP}{ZhuGP}
\newcommand{\ZhuGraphKernels}{DBLP:conf/nips/ZhuKGL04}
\newcommand{\BenDavidProvablyHelp}{DBLP:conf/colt/Ben-DavidLP08}
\newcommand{\SinghNowItHelps}{DBLP:conf/nips/SinghNZ08}
\newcommand{\TsangSparsified}{DBLP:conf/nips/TsangK06}
\newcommand{\ZhuHarmonicMixture}{DBLP:conf/icml/ZhuL05}
\newcommand{\YuBlockwise}{werfwerft}
\newcommand{\GarckeGrids}{Garcke05semi-supervisedlearning}
\newcommand{\ArgyriouEfficient}{wefqilerufh}
\newcommand{\SindhwaniLinear}{DBLP:conf/sigir/SindhwaniK06}
\newcommand{\MahdavianiRobots}{DBLP:conf/icra/MahdavianiFFH05}
\newcommand{\NadlerLimit}{NIPS2009_0465}
\newcommand{\ZhouHigherOrder}{ZhouHigherOrder}
\newcommand{\VonLuxbourgAmplified}{NIPS2010_0929}
\newcommand{\MelacciLapSVM}{LSVM_JMLR_11}

%linearSystems
\newcommand{\SpielmanNearlyLinear}{DBLP:journals/corr/abs-cs-0607105}
\newcommand{\KoutisOptimality}{DBLP:conf/focs/KoutisMP10}
\newcommand{\KoutisLinear}{DBLP:journals/corr/abs-1102-4842}

%graphs
\newcommand{\FiedlerConnectivity}{Fiedler73}

%graph learning
\newcommand{\CesaBianchiRandomSpanning}{DBLP:conf/icml/Cesa-BianchiGVZ10}

%graphicalmodels
\newcommand{\Lauritzen}{citeulike:487584}

%clustering image segmentation
\newcommand{\WuLeahy}{WuLeahy}
\newcommand{\BoumanImageModel}{Bouman93ageneralized}

%MeasureTheory
\newcommand{\DaPrato}{DaPrato}

%LearningTheory
\newcommand{\WarmuthSampleCompression}{DBLP:journals/ml/FloydW95}
\newcommand{\CuckerFoundations}{Cucker02onthe}
\newcommand{\SmolaGreens}{SmolaGreens}
\newcommand{\WolpertNoFreeLunch}{WolpertNoFreeLunch}
\newcommand{\Serfling}{Serfling}
\newcommand{\Vapnik}{Vapnik} %this is the 1998 book
\newcommand{\VapnikEstimation}{Vapnik82}
\newcommand{\VapnikUniform}{vc-ucrfep-71}
\newcommand{\MarchandSCM}{DBLP:journals/jmlr/MarchandS02}
\newcommand{\SteinwartSVMs}{Steinwart:2008:SVM:1481236}

%convex analysis
\newcommand{\FrigyikBregman}{FrigyikBregman}
\newcommand{\Zalinescu}{Zalinescu}
\newcommand{\KakadeDuality}{DBLP:journals/corr/abs-0910-0610}
\newcommand{\BregmanDivergence}{citeulike:431793}
\newcommand{\BauschkeProjections}{Bauschke97legendrefunctions}   
\newcommand{\CsiszarDivergence}{citeulike:126458}

%applications
\newcommand{\KumarSocial}{1150476}
\newcommand{\WashioDataMining}{959249}
\newcommand{\SharanBioinformatics}{citeulike:578988}
\newcommand{\CollinsNLP}{Collins01convolutionkernels}
\newcommand{\HarchaouiVision}{Harchaoui07imageclassification}
\newcommand{\BonchevChemical}{BonchevChemical}

%dimensionality reduction
\newcommand{\WeinbergerMVU}{DBLP:conf/cvpr/WeinbergerS04}
\newcommand{\BelkinEigenmaps}{BelkinEigenmaps}
\newcommand{\isomap}{citeulike:266187}
\newcommand{\LLE}{Roweis00nonlineardimensionality}

%online
\newcommand{\CesaBianchiExperts}{DBLP:journals/jacm/Cesa-BianchiFHHSW97}
\newcommand{\TewariRandomAverages}{thiswillbetewarisnipspaper}

%algorithms
\newcommand{\MarchandDLM}{DBLP:journals/jmlr/MarchandS05}

%compsci
\newcommand{\VaidyaNN}{DBLP:journals/dcg/Vaidya89}

%functional Analysis
\newcommand{\MercerTheorem}{MercerTheorem}

%inference
\newcommand{\TikhonovSolutions}{TikhonovSolutions}


%spectral clustering
\newcommand{\HeinpLaplacian}{DBLP:conf/icml/BuhlerH09}

%geometry
\newcommand{\HeinonenNonLinear}{HeinonenNonLinear}


\newcommand{\AizermanKernelTrick}{aizerman1964}
\newcommand{\ZhouDiscrete}{Zhou05regularizationon}




\newcommand{\BollobasMGT}{citeulike:150268}
\newcommand{\DiestelBook}{DIE05B}


\newcommand{\Valiant}{DBLP:conf/stoc/Valiant84}
\newcommand{\Devroye}{citeulike:134351}
\newcommand{\AnthonyBartlett}{AnthonyNeural}
\newcommand{\PredictionLearningGames}{1137817}

%PACBayes
\newcommand{\McAllesterPACBayes}{McAllesterPACBayes}
\newcommand{\GermainLinearClassifiers}{DBLP:conf/icml/GermainLLM09}
\newcommand{\MaurerNote}{DBLP:journals/corr/cs-LG-0411099}
\newcommand{\RalaivolaChromatic}{DBLP:journals/corr/abs-0909-1933}
\newcommand{\RalaivolaUStat}{DBLP:journals/corr/abs-0909-1933}
\newcommand{\BlanchardOccam}{DBLP:conf/colt/BlanchardF07}
\newcommand{\JohnAndJohn}{JohnAndJohn}
\newcommand{\LongerDDPB}{LongerDDPB}
\newcommand{\LeverDistributionDependent}{\DDPACBayes}
\newcommand{\AmbroladzeTight}{DBLP:conf/nips/AmbroladzePS06}
\newcommand{\CatoniThermodynamics}{CatoniThermodynamics}
\newcommand{\DDPACBayes}{DDPACBayes}
\newcommand{\LeverDDPACBayes}{\DDPACBayes}
\newcommand{\McAllesterModelSelection}{DBLP:journals/ml/McAllester03}
\newcommand{\SeegerGaussian}{DBLP:journals/jmlr/Seeger02}
\newcommand{\McallesterSimplified}{Mcallester03simplifiedpac-bayesian}
\newcommand{\AudibertHabilitation}{AudibertHabilitation}

%Bayesians
\newcommand{\SeegerGPForML}{DBLP:journals/ijns/Seeger04}
\newcommand{\WilliamsBarberLaplace}{DBLP:journals/pami/WilliamsB98}

%RKHS Theory
\newcommand{\WahbaSplines}{WahbaSplines}
\newcommand{\Aronszajn}{Aronszajn}

%density Estimation
\newcommand{\WestonSVMDensity}{Weston:1999:SVD:299094.299111}
\newcommand{\GirolamiDensity}{DBLP:journals/pami/GirolamiH03}
\newcommand{\HongZeroNorm}{ecs21407}
\newcommand{\ChenRegressionBased}{DBLP:journals/ijon/ChenHH10}
\newcommand{\ParzenWindow}{citeulike:3245941}

\newcommand{\CFNActive}{CFNActive}

\newcommand{\CoverThomas}{CoverThomas91}
\newcommand{\CesaBianchiUnknownGraphs}{DBLP:conf/alt/Cesa-BianchiGV09}

\newcommand{\KaariainenRelating}{KaariainenRelating}
\newcommand{\BoucheronSurvey}{BoucheronSurvey}

\newcommand{\KleinbergNetworkFailure}{DBLP:conf/soda/KleinbergSS04}

\newcommand{\MeirBayesianMixture}{DBLP:journals/jmlr/MeirZ03}


\newcommand{\MassartConcentration}{MassartConcentration}
\newcommand{\AdlerExtrema}{AdlerExtrema}
\newcommand{\BalcanSSL}{BalcanSSL}
\newcommand{\Billingsley}{Billingsley}
\newcommand{\RademacherStructure}{RademacherStructure}
\newcommand{\LeverStructure}{RademacherStructure}
\newcommand{\Krein}{Krein}

\newcommand{\TalagrandBanachSpace}{LedouxTalagrand}
\newcommand{\LedouxProbabilityInBanachSpaces}{LedouxTalagrand}
\newcommand{\KallenbergDimensionFree}{KallenbergSztencel}
\newcommand{\BenedekLearnability}{DBLP:conf/colt/BenedekI88}
\newcommand{\Decoupling}{Decoupling}
\newcommand{\HoeffdingInequalities}{citeulike:3392582}
\newcommand{\ClemenconRanking}{Clémençon}
\newcommand{\SerflingApproximation}{sterfling1980}
\newcommand{\AdamczakMoment}{Adamczak:math0506026}
\newcommand{\ArconesUProcess}{Arcones}
\newcommand{\MajorUStats}{Major}
\newcommand{\NolanUProcesses}{Nolan}
\newcommand{\McDiarmid}{McDiarmid}
\newcommand{\Massart}{Massart}

\newcommand{\HeinLaplacianConvergence}{DBLP:journals/corr/abs-math-0608522}
\newcommand{\HeinSmoothnessConvergence}{DBLP:conf/colt/Hein06}

\newcommand{\StructureBounds}{StructureBounds}
\newcommand{\MNIST}{mnistlecun}
\newcommand{\SchwarzSingerConvexGames}{DBLP:conf/nips/Shalev-ShwartzS06}
\newcommand{\RandomGraphDynamics}{Durrett}
\newcommand{\KoltchinskiPanchenko}{Panchenko00empiricalmargin}
\newcommand{\KoltchinskiiPanchenko}{Panchenko00empiricalmargin}
\newcommand{\BousquetIntroduction}{citeulike:1423736}
\newcommand{\CowellBook}{Cowell03}
\newcommand{\MackayBook}{mackay2003itila}
\newcommand{\YedidiaUnderstanding}{Yedidia_al2003BeliefPropagation}
\newcommand{\ChungComplexNetworks}{citeulike:2670734}
\newcommand{\ZhuLiteratureSurvey}{ZhuLiteratureSurvey}
\newcommand{\GoldbergDissimilarity}{Goldberg+Zhu+Wright:07a}
\newcommand{\EnumerationCospectral}{DBLP:journals/ejc/HaemersS04}



\newcommand{\GrimmetMRF}{Grimmett73atheorem}
\newcommand{\GemanGeman}{geman_stochastic_1984}
\newcommand{\Dyer}{702970}
\newcommand{\ShalevThesis}{ShalevThesis}
\newcommand{\ShaweTaylorSRM}{DBLP:journals/tit/Shawe-TaylorBWA98}
\newcommand{\KivenenPerceptronWinnow}{DBLP:journals/ai/KivinenWA97}

\newcommand{\BosquetStability}{DBLP:journals/jmlr/BousquetE02}
\newcommand{\BousquetStability}{BousquetStability}
\newcommand{\ElYanivStability}{DBLP:conf/colt/El-YanivP06}
\newcommand{\CoifmanDiffusionNIPS}{DBLP:conf/nips/NadlerLCK05}
\newcommand{\CoifmanDiffusion}{citeulike:2319922}
\newcommand{\HaagerupKhintchine}{Haagerup}
\newcommand{\BieGeneralConstraints}{DBLP:conf/sspr/BieSM04}
\newcommand{\ErikssonNormalizedCuts}{DBLP:conf/iccv/ErikssonOK07}
\newcommand{\BieConvexMethods}{DBLP:conf/nips/BieC03}
\newcommand{\JordanNormalizedCut}{Xing:CSD-03-1265}
\newcommand{\BalcanPACStyle}{DBLP:conf/colt/BalcanB05}
\newcommand{\KakadeOnlineGeneralization}{DBLP:conf/nips/KakadeT08}
\newcommand{\LanckrietLearningKernel}{DBLP:journals/jmlr/LanckrietCBGJ03}
\newcommand{\KoltchinskiRademacher}{DBLP:journals/tit/Koltchinskii01}
\newcommand{\BartlettRademacher}{DBLP:journals/jmlr/BartlettM02}
\newcommand{\BartlettLocalRademacher}{DBLP:conf/colt/BartlettBM02}
\newcommand{\KakadeLinearComplexity}{DBLP:conf/nips/KakadeST08}
\newcommand{\SSSVM}{DBLP:conf/nips/BennettD98}
\newcommand{\ChapelleLowDensity}{chapelle05semisupervised}
\newcommand{\GrandvaletEntropy}{DBLP:conf/cfap/GrandvaletB05}
\newcommand{\Zhang}{DBLP:conf/colt/Zhang05}
\newcommand{\BlumHoldOut}{DBLP:conf/colt/BlumKL99}
\newcommand{\GardnerPerceptron}{*****************}
\newcommand{\TSVM}{DBLP:conf/icml/Joachims99}
\newcommand{\TransductiveRademacher}{DBLP:conf/colt/El-YanivP07}
\newcommand{\PelckmansRademacher}{DBLP:conf/mlg/PelckmansS07}
\newcommand{\TransductiveGraphCuts}{MarginBasedGraphCuts}
\newcommand{\Hanneke}{Hanneke}
\newcommand{\Fiedler}{Fiedler73}
\newcommand{\nickthesis}{l-mbllla-89}
\newcommand{\winnow}{l-liaanla-88}
\newcommand{\LittlestoneWinnow}{\winnow}
\newcommand{\rudinreplex}{IB-E883108}
\newcommand{\bbproj}{Bauschke:1996:PAS}
\newcommand{\fabmyceil}{fm-alt-91}
\newcommand{\rkhsaron}{a-trk-50}
\newcommand{\wayfaster}{h-lamofek-01}
\newcommand{\passiveaggressive}{NIPS2003_LT21}
\newcommand{\romma}{ll-romma-01}
\newcommand{\avgmargin}{gw-lhlam-98}
\newcommand{\greville}{bg-gita-74}
\newcommand{\roseperc}{r-ppmisob-58}
\newcommand{\vonneumproj}{neumanproj}
\newcommand{\novikoff}{Novikoff:1963} %on convergence proofs for perceptrons
\newcommand{\kernperc}{fs-lmcpa-99}
\newcommand{\kerntron}{fcc-kafslps-98}
\newcommand{\smotron}{Platt99}
\newcommand{\genlarmar}{sc-frmd-99} 
\newcommand{\vapchertpr}{vc-tpr-74}
\newcommand{\boguyvap}{bgv-taomc-92}
\newcommand{\origmetpot}{abr-thpfmprl-64}
\newcommand{\vovkkern}{sgv-rrladv-98}
\newcommand{\nipsgraph}{hp-pgp-07}
\newcommand{\HerbsterPerceptron}{\nipsgraph}
\newcommand{\nicgentgen}{ccg-ogaola-04}
\newcommand{\eg}{kw-avegulp-97}
\newcommand{\vovk}{DBLP:conf/colt/Vovk90}
\newcommand{\VovkAggregatingStrategies}{\vovk}
\newcommand{\hkw}{hkw-spisglf-98}
\newcommand{\vovkregression}{nips-10:Vovk:1998}
\newcommand{\secondperc}{ccg-sopa-05}
\newcommand{\sslbook}{csz-ssl-06}
\newcommand{\clusterkern}{cws-ckssl-03}
\newcommand{\perceptron}{r-ppmisob-58}
\newcommand{\manifoldreg}{bns-mrgfrl-06}
\newcommand{\passiveagg}{cdks-opaa-06}
\newcommand{\sslrandomwalk}{SzummerJaakkola01}
\newcommand{\zhuposneg}{gzw-dsgbssc-07}
\newcommand{\predtree}{gh-fmplt-07}
\newcommand{\KernelAlignment}{cristianini-kerneltarget}
\newcommand{\ZhuProp}{zhu02learning}
\newcommand{\ZhouConsistency}{zhou03learning}
\newcommand{\SzummerRandomWalks}{szummerjaakkola01}
\newcommand{\ZhuHarmonicFunctions}{Zoubin1}
\newcommand{\DoyleSnell}{doyle-2000}
\newcommand{\robustpnormconf}{gl-rpna-99}
\newcommand{\robustpnormjourn}{DBLP:journals/ml/Gentile03a}
\newcommand{\Novikoff}{Novikoff:1963}
\newcommand{\Rosenblatt}{Rosenblatt:58}
\newcommand{\HelmboldWarmuthBatch}{helmbold95weak}
\newcommand{\Angluin}{DBLP:journals/ml/Angluin87}
\newcommand{\WeightedMajority}{littlestone89weighted}
\newcommand{\BelkinLargeGraphs}{DBLP:conf/colt/BelkinMN04}
\newcommand{\SecondOrderPerc}{!!!!!!!!}
\newcommand{\MinCut}{blum01learning}
\newcommand{\RandomisedMincuts}{blum04semisupervised}
\newcommand{\BelkinManifoldStructure}{belkin03using}
\newcommand{\ShiNormalizedCuts}{shi00normalized}
\newcommand{\snellMRF}{MRFandApps}
\newcommand{\Barzdin}{bf-pgrf-72}
\newcommand{\Cesabianchi}{1137817}
\newcommand{\Garey}{574848}
\newcommand{\Pounce}{Pounce}
\newcommand{\KleinRandic}{kr-rd-93}
\newcommand{\SmolaKondorGraphKernels}{DBLP:conf/colt/SmolaK03}
\newcommand{\BelkinManifoldRegularization}{DBLP:journals/jmlr/BelkinNS06}



\newcommand{\BNManifolds}{Belkin1}
\newcommand{\MitchellBook}{Mitchell:1997:ML}
\newcommand{\Grove}{267493}
\newcommand{\Papert}{**paper***}
\newcommand{\MinskyPapert}{MinskyPapert:69}
\newcommand{\Bregman}{citeulike:431793}
\newcommand{\CensorLent}{CensorLent}
\newcommand{\BestLinearPredictor}{944743}
\newcommand{\RobustpNorm}{\robustpnormjourn}
\newcommand{\OnlineGraph}{HerbsterOnLineGraph}
\newcommand{\KondorLafferty}{KonLaf02}
\newcommand{\DudaHartStork}{1325635}
\newcommand{\ScholkopfKernelBook}{Scholkopf2002}
\newcommand{\KernelsPatternClassification}{shawetaylor2004kernel}
\newcommand{\IntroductionToSVM}{CristianiniIntroductionSVM}
\newcommand{\ClusterKernels}{DBLP:conf/nips/ChapelleWS02}
\newcommand{\BeyondPointCloud}{PointCloud}
\newcommand{\icmlonlinegraph}{\OnlineGraph}
\newcommand{\Spines}{DBLP:conf/nips/HerbsterLP08}
\newcommand{\BianchiRandomTrees}{cesavitali}
\newcommand{\Graphtron}{ps-oallg-08}
\newcommand{\Jittat}{fk-lcorimb-08}
\newcommand{\KolmogorovFomin}{citeulike:381082}
\newcommand{\LittlestoneBatch}{LittlestoneBatch}
\newcommand{\GraepelCompression}{DBLP:journals/ml/GraepelHS05}
\newcommand{\BianchiGeneralization}{Cesa-Bianchi01onthe}
\newcommand{\BianchiImprovedGeneralization}{journals/tit/Cesa-BianchiG08}
\newcommand{\FloydCompression}{Floyd95samplecompression}
\newcommand{\LittlestoneCompression}{LittlestoneRelating}
\newcommand{\pInterpolation}{pInterpolation}
\newcommand{\Azuma}{azuma}
\newcommand{\Chvatal}{Chvatal}
\newcommand{\Derbeko}{Derbeko04explicitlearning}
\newcommand{\NicoloBook}{1137817}
\newcommand{\grady}{DBLP:conf/cvpr/SingarajuGV09}
\newcommand{\SpielmanLectures}{******************************}
\newcommand{\ChungBook}{ChungBook}
\newcommand{\JerrumSinclair}{***************} %the paper proving cheeger's inequality for graphs
\newcommand{\Guattery}{Guattery98onthe}
\newcommand{\PACMDL}{blum03pacmdl}
\newcommand{\LangfordTutorial}{Langford2005}
\newcommand{\ChapelleTransductiveRegression}{Chapelle99transductiveinference}
\newcommand{\SpectralGraphTransducer}{Joachims/03a}
\newcommand{\Rockafellar}{RockafellarConvexAnalysis}
\newcommand{\DhillonTropp}{Dhillon}


==> environments.tex <==
%you cannot use this if you are using COLT style file, they are defined in there. you will have to add what is missing individually

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\newenvironment{definition}[1][Definition]{\begin{trivlist}\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
